How Can Datacenters Join the Smart Grid to Address the Climate Crisis? Using simulation to explore power and cost effects of direct participation in the energy market

Amidst the climate crisis, the massive introduction of renewable energy sources has brought tremendous challenges to both the power grid and its surrounding markets. As datacenters have become ever-larger and more powerful, they play an increasingly significant role in the energy arena. With their unique characteristics, datacenters have been proved to be well-suited for regulating the power grid yet currently provide little, if any, such active response. This problem is due to issues such as unsuitability of the market design, high complexity of the currently proposed solutions, as well as the potential risks thereof. This work aims to provide individual datacenters with insights on the feasibility and profitability of directly participating in the energy market. By modelling the power system of datacenters, and by conducting simulations on real-world datacenter traces, we demonstrate the substantial financial incentive for individual datacenters to directly participate in both the day-ahead and the balancing markets. In turn, we suggest a new short-term, direct scheme of market participation for individual datacenters in place of the current long-term, inactive participation. Furthermore, we develop a novel proactive DVFS scheduling algorithm that can both reduce energy consumption and save energy costs during the market participation of datacenters. Also, in developing this scheduler, we propose an innovative combination of machine learning methods and the DVFS technology that can provide the power grid with indirect demand response (DR). Our experimental results strongly support that individual datacenters can and should directly participate in the energy market both to save their energy costs and to curb their energy consumption, whilst providing the power grid with indirect DR.

==> chapters/6-related-work/6.1_dsm.tex <==
\section{Demand Side Management} \label{sec:dsm}

Intensive work have been conducted to explore datacenter’s participation in DSM programmes. A synergistic control strategy and a flexibility factor have been developed to increase the capacity of frequency regulation in a recent study \cite{Fu2020AssessmentsOD}. \citeauthor{Fu2020MultimarketOO} present a real-time, multi-market optimization framework for the datacenters without storage systems to maximize \cite{Fu2020MultimarketOO}, facilitating datacenters to participate in both the in the both the energy market and the regulation market. Taking into account the energy cost, demand costs and regulation revenues, the framework optimizes the bid in each hour, helping datacenters meet energy and demand goals whilst keep minimum cost through obtaining maximum regulation revenues. However, these work focuses on enlarging the FR capacity of datacenters, which is of rarity in the industry \cite{Bates2014ElectricalGA}.

Via dynamic pricing, \citeauthor{Li2013TowardsDP} propose a collaborative framework for optimizing the overall costs of several datacenters in their position paper \cite{Li2013TowardsDP}. The framework employ collaborative efforts across multiple geographically distributed datacenters communicated via dedicated network fabric to negotiate a mutually optimal energy price. In this collaborative system, an optimization platform \cite{Liu2012CologneAD} is used to enable constraint optimization problems (COPs). However, to benefit from these schemes, multiple datacenters and their utility companies have to be involved to optimize the price update in the energy market.

In terms of market design, two categories of programmes for DR are commonly available. The first category involves biding/supplying a certain amount of demand flexibility in to the market. In other words, consumers bid their flexibility via supply functions that are parameterized (\eg \cite{Johari2011ParameterizedSF,Xu2016DemandRW}). In the second category, consumers buy in/response to published prices that were selected according to predictions on potential available flexibility. Examples of the second sort include \cite{Conejo2010RealTimeDR,
Li2011OptimalDR,Rad2010OptimalRL,Liu2014PricingDC}. Specifically, programmes such as the Coincident Peak Pricing (CPP) \cite{Baldick2018IncentivePO} and price-based incentive programmes \cite{Sle2011DemandRF} are available for datacenters to participate. These programmes charge much higher prices for electricity during peak hours (usually over 200$\times$ more expensive than the base price \cite{Liu2014PricingDC}). Such peak-hour costs can account for 23+\% of the consumers’ energy bill \cite{peak_bill}, which is a strong motive for consumers to reduce their energy usage during peak hours. However, when it comes to datacenters, \citeauthor{Liu2014PricingDC} argue that the market designs and models in the second category outperform that in the first. Also, the current available DR programmes, such as CPP, are not particularly suitable for datacenters since they can barely fully utilize the flexibility of datacenters due to many reasons. Chief amongst them is that although datacenters may incur charges if no response is offered, no profit would be produced either if the peak in energy load does not happen during the coincident periods. As a result, datacenters nowadays provide little, if any, response to market signals \cite{Ghatikar2012DemandRO,glanz2012power,Liu2014PricingDC,Liu2013DataCD}. In addition, a large amount of efforts has been devoted to the optimization of workload management of datacenters (\eg \cite{Chen2010IntegratedMO,Gandhi2011MinimizingDC,Heo2011OptiTunerOP,Lin2011DynamicRF,Meisner2011PowerMO,Xu2012CostED,Yao2012DataCP,Zhang2012DynamicEC}), especially, via workload distribution \cite{Rao2010MinimizingEC,Liu2015GreeningGL,Ghamkhari2013EnergyAP,Wang2012DProDD,Zhang2015ATI,Wang2016ProactiveDR}. If this is considered, time for shedding the load can be saved and, in turn, the flexibility of datacenters can be further increased. Moreover, by exploiting the regional difference of the energy cost, datacenters can leverage their distributed nature to further optimized \cite{Qureshi2009CuttingTE,Rao2010MinimizingEC,Liu2015GreeningGL,Lin2012OnlineAF,Ghamkhari2013EnergyAP,Wang2012DProDD,Zhang2015ATI}. Nevertheless, such these management strategies require cooperation between the power grid and geographically distributed datacenters together with their utility companies. Thus, they far more complex to orchestrate than what is introduced in this work, which would potentially hinder their adoption. 

==> chapters/6-related-work/6.2_simulation.tex <==
\section{Datacenter Energy Simulation} \label{sec:simulator}



==> chapters/6-related-work/6_related_work.tex <==
\chapter{Related Work (Move to Background)} \label{cha:related_work}

introduction goes here ...

\input{chapters/6-related-work/6.1_dsm}

\input{chapters/6-related-work/6.2_simulation}

\section{ML Forecast in the Energy Market}

==> chapters/backup.tex <==
\chapter{Test}

\section{Balancing System}

\newpage
\begin{table}[H]
    \centering
    \begin{tabular}{ll}
    \toprule
        $p^S$ & Spot market price \\
        $p^B_-$ & Shortage price in the balancing market \\
        $p^B_+$ & Surplus price in the balancing market \\
        $Q_-$ & Quantity of shortage energy of a BRP \\
        $Q+$ & Quantity of surplus energy of a BRP \\
        $Q+$ & Quantity of energy required by downwards regulations \\
        $Q_\downarrow$ & Quantity of energy required by downwards regulations \\
        $Q_\uparrow$ & Quantity of energy required by upwards regulations \\
        $N_\text{BSP}$ & Number of participated BSPs in the balancing market \\
        $N_\text{BRP}$ & Number of participated BRPs in the balancing market \\
    \bottomrule
    \end{tabular}
    \caption{Nomenclature.}
    \label{tab:sym_load}
\end{table}

One-price system:
\begin{align}
&\mathlarger{
    \sum^{N_\text{BSP}}_i \left(  Q_{\downarrow_i} \cdot p^B_\downarrow \right) + 
        \sum^{N_\text{BRP}}_j \left(  Q_{-_j} \cdot p^B_- \right)
} \nonumber \\
&\hspace{0.3\textwidth} \mathlarger{=} \\
&\mathlarger{
    \sum^{N_\text{BSP}}_i \left(  Q_{\uparrow_i} \cdot p^B_\uparrow \right) + 
        \sum^{N_\text{BRP}}_j \left(  Q_{+_j} \cdot p^B_+ \right)
} \nonumber
\end{align}

\noindent Two price system:
\begin{align}
&\mathlarger{
    \sum^{N_\text{BSP}}_i \left(  Q_{\downarrow_i} \cdot p^B_\downarrow \right) + 
        \sum^{N_\text{BRP}}_j \left(  Q_{-_j} \cdot p^B_- \right)
} \nonumber \\
&\hspace{0.3\textwidth} \mathlarger{=} \\
&\mathlarger{
    \sum^{N_\text{BSP}}_i \left(  Q_{\uparrow_i} \cdot p^B_\uparrow \right) + 
        \sum^{N_\text{BRP}}_j \left(  Q_{+_j} \cdot p^S \right)
} \nonumber
\end{align}

\newpage
\section{Load Scheduling}
\begin{table}[H]
    \centering
    \begin{tabular}{ll}
    \toprule
        $l$ & Load of the next day \\
        $q$ & Quantile to apply \\
        $s$ & Scalar to apply \\
        $Q^S$ & Quantity of energy to order in the spot market \\
    \bottomrule
    \end{tabular}
    \caption{Nomenclature.}
    \label{tab:sym_load}
\end{table}

\begin{equation}
% \mathlarger{
    Q^S = \mathbb{Q}_q(l) \cdot s, \quad q \in [0, 1]\ \text{and}\ s \in [0.97, 1.30]
% }
\end{equation}

\newpage
\section{AA Metric}

\begin{table}[H]
    \centering
    \begin{tabular}{ll}
    \toprule
        $N_\text{ISP}$ & Number of ISPs\\
        $p^S$ & Spot price in the day-ahead market \\
        $p^B$ & Shortage price in the balancing market \\
        $p^F$ & Forecasted imbalance price. \\
        $p^f$ & Synthetically forecast price. \\
        $E$ & Additive Gaussian random variable. \\
    \bottomrule
    \end{tabular}
    \caption{Nomenclature.}
    \label{tab:sym_aa}
\end{table}

\begin{equation}
    \mathbb{S}(x) = 
        \begin{cases}
            +1 & x > 0\\
            0 & x = 0\\
            -1 & x <0
        \end{cases}
\end{equation}

Agreement accuracy ($AA$):
\begin{equation}
\mathlarger{
    AA = \cfrac{ \sum^{N_\text{ISP}}_{i} 
                \mathlarger{\mathds{1}\left\{
                    \mathds{1}\left[\mathbb{S}(p_i^B) = \mathbb{S}(p_i^F)\right]
                    = 
                    \mathds{1}\left[\mathbb{S}(p_i^B - p_i^S) = \mathbb{S}(p_i^F - p_i^S) \right]
                    \right\}}
            } 
             {N_\text{ISP}}
}
\end{equation}

where $N_\text{ISP}$ is the number of ISPs, $p^S$ is the spot price in the day-ahead market, $p^B$ is the shortage price in the balancing market, and $p^F$ is the predicted imbalance price.

\subsection{Synthetic Forecast}

\begin{equation}
\mathlarger{
    p^f = p^B + E, \quad E \sim \mathlarger{\mathcal{N}}(0, \sigma) = \cfrac{1}{{\sigma \sqrt {2\pi } }}\cdot e^{-\frac{1}{2} \left(\frac{x}{\sigma}\right)^2}
}
\end{equation}

\newpage

\section{Support Power Model}
\begin{table}[H]
    \centering
    \begin{tabular}{ll}
    \toprule
    %   $P^\text{\ in}$  & Inlet power & 
      $\pi$ & Nameplate loss coefficient \\
    %   $P^\text{\ out}$ & Outlet power & 
      $\lambda$ & Tare loss coefficient \\
      $\alpha$ & Proportional loss coefficient \\
      $\beta$ & Square-law loss coefficient \\
      $P^\text{\ in}$  & Inlet power \\
      $P^\text{\ tare}$ & Tare power loss \\
      $P^\text{\ loss}$ & Total power loss \\
      $P^\text{\ rated}$ & Nameplate power \\
      $P^\text{2nd}$ & Power draw of secondary power support\\
      $N_\text{\ server}$ & Number of active servers \\
      $N_\text{\ PDU}$ & Number of attached PDUs \\
    \bottomrule
    \end{tabular}
    \caption{Nomenclature.}
    \label{tab:sym_support}
\end{table}

\begin{equation}
    \begin{cases}
    \alpha = \pi_\text{\ UPS} - \lambda_\text{\ UPS} \\
    \\
    P^\text{\ tare}_\text{\ UPS} = \lambda_\text{\ UPS} \cdot P^\text{\ rated}_\text{\ UPS} \\
    \\
    P^\text{\ loss}_\text{\ UPS} = P^\text{\ tare}_\text{\ UPS} + \alpha \cdot (\sum^{N_\text{\ PDU}}_{i} P^\text{\ in}_{\text{\ PDU}_i})
    \end{cases}
    \label{eq:ups}
\end{equation}

\begin{equation}
    \begin{cases}
    \beta = \pi_\text{\ PDU} - \lambda_\text{\ PDU} \\
    \\
    P^\text{\ tare}_\text{\ PDU} = \lambda_\text{\ PDU} \cdot P^\text{\ rated}_\text{\ PDU} \\
    \\
    P^\text{\ loss}_\text{\ PDU} = P^\text{\ tare}_\text{\ PDU} + \beta \cdot (\sum^{N_\text{\ server}}_{i} P^\text{\ in}_{\text{\ server}_i})^2
    \end{cases}
    \label{eq:pdu}
\end{equation}

\subsection{Secondary support}

\begin{equation}
    P^\text{2nd} = \text{PUE} \cdot (\sum^{N_\text{\ server}}_{i} P_{\text{\ server}_i} + \sum^{N_\text{\ PDU}}_{i} P_{\text{\ PDU}_i} + \sum^{N_\text{\ UPS}}_{i} P_{\text{\ UPS}_i})
\end{equation}


==> resources/tables/tab_experts.tex <==
\begin{table}[H]
\centering
\begin{adjustbox}{width=\textwidth}

    \begin{tabular}{c|l|l}
    \toprule
        \textbf{Industry} & \textbf{Role} & \textbf{Size of Infrastructure Dealt w/}\\
        \midrule
        Energy            & Machine Learning Engineer & Large\\
        IT                & Engineer and Scientist    & Medium\\
        IT                & Researcher                & Medium \& Small \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption[Experts involved in requirement verification and validation]{Experts involved in requirement verification and validation.}
\label{tab:experts}
\end{table}
